Buddy-RAM: Improving the Performance and Efficiency of Bulk Bitwise Operations Using DRAM

Bitwise operations are an important component of modern day programming. Many widely-used data structures (e.g., bitmap indices in databases) rely on fast bitwise operations on large bit vectors to achieve high performance. Unfortunately, in existing systems, regardless of the underlying architecture (e.g., CPU, GPU, FPGA), the throughput of such bulk bitwise operations is limited by the available memory bandwidth. We propose Buddy, a new mechanism that exploits the analog operation of DRAM to perform bulk bitwise operations completely inside the DRAM chip. Buddy consists of two components. First, simultaneous activation of three DRAM rows that are connected to the same set of sense amplifiers enables us to perform bitwise AND and OR operations. Second, the inverters present in each sense amplifier enables us to perform bitwise NOT operations, with modest changes to the DRAM array. These two components make Buddy functionally complete. Our implementation of Buddy largely exploits the existing DRAM structure and interface, and incurs low overhead (1% of DRAM chip area). Our evaluations based on SPICE simulations show that, across seven commonly-used bitwise operations, Buddy provides between 10.9X---25.6X improvement in raw throughput and 25.1X---59.5X reduction in energy consumption. We evaluate three real-world data-intensive applications that exploit bitwise operations: 1) bitmap indices, 2) BitWeaving, and 3) bitvector-based implementation of sets. Our evaluations show that Buddy significantly outperforms the state-of-the-art.

==> spice.tex <==
\subsection{SPICE Simulations}
\label{sec:spice-sim}

We perform SPICE simulations to confirm the reliability of
\tra. We implement the DRAM sense amplifier circuit using 55nm
DDR3 model parameters~\cite{rambus}, and PTM low-power transistor
models~\cite{ptmweb,zhaoptm}. We use cell/transistor parameters
from the Rambus power model~\cite{rambus} (cell capacitance =
22fF, transistor width = 55nm, transistor height = 85nm).

The DRAM specification is designed for the worst case conditions
when a cell has not been accessed for a long time (refresh
interval). Therefore, we can activate a fully refreshed cell with
a latency much lower than the standard activation latency,
35ns~\cite{charge-cache,nuat}. In fact, we observe that we can
activate a fully charged/empty cell in 20.9~ns/13.5~ns.

For \tra, there are four possible cases depending on the number
cells that are initially fully charged. For these cases, we add
different levels of process variation among cells, so that the
strong cell attempts to override the majority decision of the two
weak cells. Table~\ref{tab:pv} shows the latency of \tra for the
four possible cases with different levels of process variation,
where \emph{s} and \emph{w} subscripts stand for \emph{strong}
and \emph{weak}, respectively, for the cells that store either 0
or 1.  

\begin{table}[b]\footnotesize
  \centering
  \input{tables/pv}
  \caption{Effect of process variation on the latency of
    triple-row activation. All times are in ns.}
  \label{tab:pv}
\end{table}

We draw three conclusions. First, for the cases where all three
cells are either 0 or 1, the latency of \tra is stable at around
16~ns and 22~ns respectively, even in the presence of process
variation. This is because, in these two cases, all three cells
push the bitline toward the same direction. Second, for the other
two cases, while the latency of \tra increases with increasing
process variation, it is still well within the DRAM specification
even with $\pm$20\% process variation (i.e., \emph{a 40\%
difference in cell capacitance}). Third, we observe the first
failure at $\pm$25\% for the $1_s0_w0_w$ case. In this case,
the sense amplifier operates incorrectly by detecting a ``1''
instead of ``0''. In summary, our SPICE simulations show that
\tra works as expected even in the presence of significant
process variation.


Prior works~\cite{al-dram,data-retention,vrt-1,vrt-2} show that
temperature increases DRAM cell leakage. However, as we show in
the next section, our mechanism \emph{always} ensures that the
cells involved in the TRA are fully refreshed just before the
operation. Therefore, we do not expect temperature to affect the
reliability of TRA.


